Anatomy-Aware Cardiac Motion Estimation

Cardiac motion estimation is critical to the assessment of cardiac function. Myocardium feature tracking (FT) can directly estimate cardiac motion from cine MRI, which requires no special scanning procedure. However, current deep learning-based FT methods may result in unrealistic myocardium shapes since the learning is solely guided by image intensities without considering anatomy. On the other hand, motion estimation through learning is challenging because ground-truth motion fields are almost impossible to obtain. In this study, we propose a novel Anatomy-Aware Tracker (AATracker) for cardiac motion estimation that preserves anatomy by weak supervision. A convolutional variational autoencoder (VAE) is trained to encapsulate realistic myocardium shapes. A baseline dense motion tracker is trained to approximate the motion fields and then refined to estimate anatomy-aware motion fields under the weak supervision from the VAE. We evaluate the proposed method on long-axis cardiac cine MRI, which has more complex myocardium appearances and motions than short-axis. Compared with other methods, AATracker significantly improves the tracking performance and provides visually more realistic tracking results, demonstrating the effectiveness of the proposed weakly-supervision scheme in cardiac motion estimation.

==> back_info.tex <==
%Cardiac MRI feature tracking (CMR-FT) has thus raised much attention recently \cite{tsadok2013automatic,bai2018automated,puyol2018fully,heinke2019towards}. In CMR-FT, time-varying cardiac motion is estimated from cine MRI that usually includes a complete cycle of cardiac contraction and relaxation, as shown in Fig. \ref{fig:cineMRI_cardiac_cycle}. 
% where anatomically realistic shapes are estimated via enforcing anatomical constraints \cite{mansilla2020learning} 
% The 2D segmentation model can hardly make use of the temporal information between neighboring frames. Also, holes and islets can appear in the segmentation results. 3D segmentation model inherently captures temporal information in cine MRI. Nevertheless, the annotation burden is substantial, and the training requires a large amount of GPU memory. Moreover, segmentation-based CMR-FT methods is a multiple-stage framework.
%Then the source image becomes a new reference frame, and the motion occurred next is estimated. The process continues for all the consecutive frames, and motion for the full cardiac cycle is obtained.
% sokooti2017nonrigid
%  and achieves state-of-the-art in many applications
% Moreover, with GPU-accelerated computing, the time consumption of CNN-based registration decreases significantly comparing to conventional methods.
% We take advantage of the CNN-based unsupervised image registration and adapt it to be symmetric as the baseline model for CMR-FT \cite{jaderberg2015spatial,balakrishnan2018unsupervised}. With this model, we compose the registration flow fields between consecutive frames to form the flow fields for the first frame with all the rest in cine MRI. Besides, we propose a flow refining mechanism on the flow comprising process to boost the baseline tracking performance.
% Image-based unsupervised registration for CMR-FT achieves promising myocardium overlapping with the ground truth, measured by the Dice similarity coefficient (DSC).
% Painchaud \textit{et al.} proposed a post-processing procedure to warp anatomically inaccurate tracked shapes to plausible ones. 
% employ an adversarial variational autoencoder (aVAE) as a post-processing procedure  \cite{painchaud2019cardiac}.
% convolutional variational autoencoder to refine anatomy boundaries \cite{painchaud2019cardiac,mansilla2020learning}.  Besides, Mansilla \textit{et al.} enforce the global agreement between deformed source mask with target segmentation mask through minimizing the difference of their VAE encoded latent space to learn constrained deformable model \cite{mansilla2020learning}. Nevertheless, all images' masks are required to enforce the constraints.
% \cite{higgins2017beta,zhang2019d}
% the warped mask to be the same as the VAE refined myocardium. We constrain the motion estimation further via enforcing the warped mask to be also close to its VAE reconstruction. Fig. \ref{fig:motion_estimation} presents the diagram of the baseline model and the shape-constrained motion estimation model with the consideration of preserving anatomy for CMR-FT. 
%Before deep learning, deformable models, such as free-form deformation (FFD) \cite{rohlfing2003volume,ledesma2005spatio,heyde2012three,lorenzi2013lcc} achieve leading performance. 
%Deep learning, given its huge success in other computer vision tasks \cite{krizhevsky2012imagenet,lecun2015deep}, has been applied to motion estimation as well \cite{qin2018joint,de2019deep,krebs2019learning,morales2019implementation}. 
%Deep learning has been applied to motion estimation as well \cite{qin2018joint,de2019deep,krebs2019learning,morales2019implementation}. 
% We conduct a further registration from $\mathcal{I}_{n}^{'}$ to $\mathcal{I}_{n}$ and obtain another flow, denoted as $f_{n}^{\delta}$. We refine the flow field between the first frame and the $n$-th frame by further composing $\mathcal{F}_{1n}$ with $f_{n}^{\delta}$ to attain the final flow $\mathcal{F}_{1n}^{*}$. Next, we track the $n$-th myocardium mask via warping the first frame mask based using $\mathcal{F}_{1n}^{*}$ to evaluate the motion estimation.

% In the context of CMR-FT, left ventricle (LV) myocardium is usually the object of interest and is tracked through time. Myocardium semantic information (i.e. segmentation mask) at the first frame (end of diastole ED) is given either by cardiologists' annotation or computer-aided algorithms. Given such segmentation mask, we utilize the motion estimation network to track the myocardium through the entire video.  
%a motion flow field generation decoder based on the concatenation of up-sampled feature maps from different feature abstraction levels, 
%With the capability of motion estimation from two images, we can now perform CMR-FT for cine MRI. 
%Fig. \ref{fig:myocardium_tracking}(A) summarizes the myocardium feature tracking process. 
%With these consecutive frame motion fields, we compute the composite flow field $\hat{\mathcal{F}}_{1n}$ between the first frame and the n-th frame as:
%Two points are worth mentioning here: first, 
%Examples can be found in ``Tracked Masks" row in Fig.~\ref{fig:myocardium_tracking}. 
%The input of VAE is myocardium mask and the output is the reconstructed mask. The VAE model is trained on available myocardium annotations. 
%%In the following, we explain an improved motion estimation method considering shape constraint by utilizing the trained VAE model.
%we first use the baseline model to feature-track the myocardium so that every image has a corresponding coarse segmentation of the myocardium. 
% so that $\mathcal{M}_{1}^{'}$ and $\mathcal{M}_{2}^{'}$ approximate to corrected shapes $\mathcal{M}_{1}$ and $\mathcal{M}_{2}$ respectively. We use $\ell_{1}$-norm to compute the difference and we have the loss function as
%We randomly select $80\%$ movies as the training set. We further randomly select 45 movies from the remaining $20\%$ data for both 2- and 4-chamber and fully annotate their myocardium for the final evaluation. We use the rest cine MRIs for validation. Besides, we randomly select 300 cine MRIs from the training set and annotate their first frame's myocardial mask and use for the shape-constrained motion estimation refining.
%  and obtain 909 and 888 cine MRI samples for 2- and 4-chamber
% The raw cine MRIs in the Kaggle dataset have different physical and image resolutions. We first rescale cine MRIs to the same physical resolution. Then we crop images with a size of $192\times192$. The myocardium masks are annotated based on the raw cine MRIs with the same scaling and cropping. We further normalize the cropped image by subtracting its mean and dividing by its standard deviation.
% and take it as the input for the registration model and the tracking process.
%Since we cannot directly evaluate the estimated motion field because lack of ground truth motion field, we evaluate the motion estimation model based on the tracked myocardium. 
% thus to be a proper metric for myocardium boundary anatomy preserving.
% In the baseline model, we use Adam optimizer with a learning rate of 1.0e-4. We train the model for five epochs with a batch size of 16 and set $\lambda_{H}$ as 0.02. 
% Adam optimizer, with an initial learning rate of 1.0e-4, is applied to train the VAE model. The learning rate decays in an epoch-wise step-down manner until 0.0. We train the VAE model for 1000 epochs with a batch size of 32. 
% We set the learning rate as 5.0e-6 and the batch size as 16. 
% We fine-tune the motion estimation model for one epoch and save it as the final model. %We implement all these models using PyTorch.E and set the latent space as a 32-d representation. We set $\lambda_{I}$, $\lambda_{fake}$, $\lambda_{recon}$, and $\lambda_{H}$ as 0.5, 3.0, 0.6, 0.02, respectively.

%The implementation includes baseline m
%  However, FFD has close HD values with the baseline model. 
%%Besides the reconstruction loss presented here, we have also explored other ways to add shape constraints, such as enforcing the consistency between the tracked and the VAE reconstructed masks in the latent space, and enforcing the zero motion field between the two. We find the proposed the method achieves the best performance. 
% In addition, we can also  Furthermore, instead of $\ell_{1}$-norm on the myocardium mask, we can also apply the $\ell_{2}$-norm for the constraints loss. From our experiments, the myocardium mask-based obtains the best performance compared with constraints on flow or VAE latent space. As for the $\ell_{1}$-norm and $\ell_{2}$-norm, the $\ell_{2}$-norm obtains better DSC but higher HD, and we choose $\ell_{1}$-the norm for anatomy preserving.


% As we can see in Fig. \ref{fig:patient_wise_cmp}, there exist several cases obtaining even higher HD and ASSD after the motion estimation refinement. Some explanations needed here.
% , and the overall model is trained for one epoch and saved as the final model
%We can also observe the improved performance of the anatomy-aware model over baseline in Fig.~\ref{fig:patient_wise_cmp} and in examples in Fig.~\ref{fig:myocardium_mask_cmp}. 

%To solve this problem, we enforce a myocardium shape constraint (anatomy-awareness) in the motion estimation. In this work, we utilize convolutional VAE \cite{pu2016variational,hou2017deep,higgins2017beta} to encode myocardium anatomy structure. 

% All models are trained with Adam optimizer with scheduled learning rate decay.

% We only annotate myocardial masks on the first frame of each cine MRI in the training data but all frames in the testing data.
%%Some studies have proposed to introduce shape prior knowledge by variational autoencoder (VAE). For example, Painchaud \textit{et al.} employ VAE as a post-processing procedure to warp anatomically inaccurate tracked shapes to plausible ones \cite{painchaud2019cardiac}.
% $90^\circ$, $180^\circ$, and $270^\circ$ followed by random rotation in the range -$45^\circ$ to $45^\circ$,

% Some studies estimate motions directly from images \cite{wu2014s,de2017end,balakrishnan2018unsupervised,mansilla2020learning}.  Nevertheless, learning-based CMR-FT motion estimation is inherently challenging since it is difficult to obtain ground truth motion, and many studies formulate the task in an unsupervised scheme \cite{balakrishnan2018unsupervised,de2019deep}. Because myocardium has similar image appearances with neighboring tissues/organs such as the papillary muscle, mere image-based motion estimation will face severe ambiguity in these regions, which causes anatomically unrealistic tracked results. 
 % \cite{chandrashekara2004analysis,pan2005fast,mansi2009physically,%shi2012comprehensive,shi2013temporal}. 
 
 %%The reason behind of utilizing segmentation is that the segmentation regularizes myocardium tracking and reduces tracking disturbances caused by neighbouring organs or artifacts.

%The estimated motion field is used to help segmentation task.

 
% In general motion estimation task, deformable models, such as  , have achieved leading performance but later are surpassed by deep learning methods \cite{,de2019deep,krebs2019arning,morales2019implementation}. Nevertheless, learning-based motion estimation is inherently challenging since it is difficult to obtain ground truth motion, and many studies formulate the task in an unsupervised scheme \cite{balakrishnan2018unsupervised,de2019deep}.

% We perform extensive augmentation to improve the robustness of the VAE model. 
% Eric: will re-write the above paragraph later. 
% Note that we only use the 300 cine with first frame annotation for AATracker training, and these data have no overlap with those 100 cine MRI (3,000 frames) used for the VAE training.
